Tree-level soft emission of a quark pair in association with a gluon

We compute the tree-level current for the emission of a soft quark-antiquark pair in association with a gluon. This soft current is the last missing ingredient to understand the infrared singularities that can arise in next-to-next-to-next-to-leading-order (N$^3$LO) computations in QCD. Its square allows us to understand for the first time the colour correlations induced by the soft emission of a quark pair and a gluon. We find that there are three types of correlations: Besides dipole-type correlations that have already appeared in soft limits of tree-level amplitudes, we uncover for the first time also a three-parton correlation involving a totally symmetric structure constant. We also study the behaviour of collinear splitting amplitudes in the triple-soft limit, and we derive the corresponding factorisation formula.

==> app_collinear_kinematics.tex <==
%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%
\section{Kinematics of the collinear limit}
\label{app:boost}

In this appendix, we examine the kinematics of the


We use a generic light-cone decomposition of $m$ massless momenta,
%
\begin{equation} 
\label{eq:collinear_app1}
p_i^\mu = x_i\pM{\mu} + k_{\perp i}^\mu + a_i n^\mu\,, \qquad i=1,\ldots,m\,,
\end{equation}
%
where the light-like momentum,
%
\begin{equation}
\pM{} = ( \sqrt{ ({\bf p}_1+\ldots + {\bf p}_m)^2}, {\bf p}_1+\ldots + {\bf p}_m )\,,
\label{eq:collinear_app2}
\end{equation}
%
specifies a light-cone direction, $\pM{} \cdot k_{\perp i} = 0$,
$n^\mu$ is an auxiliary light-like vector, which specifies how that light-cone direction is approached, $n\cdot k_{\perp i} = 0$,
and $x_i$ are the longitudinal momentum fractions with respect to the total momentum $P^\mu = \sum_{i=1}^m p_i^\mu$.
Note that
%
\begin{equation} 
\label{eq:collinear_app3}
x_i = \frac{p_i\cdot n}{\pM{} \cdot n}\,, \qquad  a_i = \frac{p_i\cdot \pM{}}{\pM{}\cdot n }\,,
\qquad i=1,\ldots,m\,,
\end{equation}
%
and the on-shellness condition, $p_i^2 = 0$, allows us to fix
%
\begin{equation} 
\label{eq:collinear_app4}
a_i = - \frac{k_{\perp i}^2}{2x_i \pM{}\cdot n}\,,
\end{equation}
%
so we arrive at the usual expression in eq.~(\ref{eq:collinear_momenta}) for the light-cone decomposition.

Note that eq.~(\ref{eq:collinear_app3}) implies that
%
\begin{equation} 
\label{eq:collinear_app5}
\sum_{i=1}^m x_i = \frac{P\cdot n}{\pM{} \cdot n} \ne 1\,,
\end{equation}
%
and
%
\begin{equation} 
\label{eq:collinear_app6}
\sum_{i=1}^m p_i^\mu = P^\mu = \frac{P\cdot n}{\pM{} \cdot n} \pM{\mu} + 
\sum_{i=1}^m k_{\perp i}^\mu + \frac{P\cdot \pM{}}{\pM{} \cdot n} n^\mu\,,
\end{equation}
%
which shows that in general $\sum_{i=1}^m k_{\perp i}^\mu \ne 0$.
Only in the strict collinear limit ${f \to f_1\ldots f_m}$, for which $P^\mu\to \pM{\mu}$, are the constraints
$\sum_{i=1}^m x_i =1 $ and $\sum_{i=1}^m \K{i}^\mu = 0$ fulfilled.

However, the longitudinal-boost invariant variables,
%
\begin{equation}
z_i = \frac{x_i}{\sum_{j=1}^m x_j} = \frac{p_i\cdot n}{P\cdot n}\,, 
\qquad 
\KT{i}^\mu = \K{i}^{\mu}- z_i\sum_{j=1}^m \K{j}^{\mu}\,,
\label{eq:boostapp}
\end{equation}
%
satisfy the constraints, $\sum_{i=1}^m z_i =1$ and $\sum_{i=1}^m\KT{i}^\mu= 0$ also away from the strict collinear limit.


\iffalse
For instance, the triple collinear limit involves a $(1\to 2)$ subcurrent $J^{(12)\mu}$ 
and one may define longitudinal-boost invariant quantities of the $(12)$ direction.
Decomposing then the momenta $p_i$ with respect to the directions  $(123)$ and $(12)$, it is possible to connect boost-invariant quantities in those directions. For example,
%
\begin{equation}
z_i^{(12)} = \frac{p_i\cdot n}{p_{12} \cdot  n} \equiv \frac{z_i^{(123)}}{z_1^{(123)}+z_2^{(123)}},
\qquad \tilde{k}_i^{(12)\mu} = k_{\perp i}^{\mu}- z_i^{(12)} k_{\perp 12}^{\mu}, \quad i=1,2,3,
\end{equation}
%
where 
%we have included the projection along the triple collinear direction $(123)$. Note that the parton $a_3$ too has a longitudinal momentum fraction in the $(12)$ direction. From now on, dropping 
we have added a superscript to the boost-invariant variables to label the direction of a specific subset of the $m$ collinear partons.
%shall implicitly denote the direction of the total momentum ($1\ldots m$) of $m$ final state partons.
\fi
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



==> app_colour_id.tex <==
\section{Colour identities of the multi-soft current}
\label{app:colour_identities}

In this appendix we recall the
colour identities~\cite{Czakon:2011ve} which are relevant in the derivation of the three- and four-parton colour correlations of the soft-$q\bar{q}g$ current.

The identity,
%
\begin{align}
    if^{abc}\left[\left\{\mathbf{T}_i^a,\mathbf{T}_j^b\right\},\mathbf{T}_k^c\right] =
    2C_A \mathbf{T}_i\cdot\mathbf{T}_j(\delta_{ik}-\delta_{jk})\,, \nonumber
\end{align}
%
has been introduced in \eqn{eq:dipcol}.
The identity,
\iffalse
\begin{align}
    \begin{split}
    &\left\{\left\{\mathbf{T}_i^{a},\mathbf{T}_j^{b}\right\},\left\{\mathbf{T}_k^{a},\mathbf{T}_l^{b}\right\}\right\}
    %+\left\{\left\{\mathbf{T}_i^{a},\mathbf{T}_l^{b}\right\},\left\{\mathbf{T}_k^{a},\mathbf{T}_j^{b}\right\}\right\} 
    +(j\leftrightarrow l)\\
    &\qquad=
    8\{\mathbf{T}_i\cdot\mathbf{T}_k,\mathbf{T}_j\cdot\mathbf{T}_l\}
    +2C_A\big(
    3\delta_{il}\delta_{jk}\mathbf{T}_i\cdot\mathbf{T}_j 
    + 3\delta_{ij}\delta_{kl}\mathbf{T}_i\cdot\mathbf{T}_k \\
    &\qquad-2\delta_{ij}\delta_{jk}\mathbf{T}_i\cdot\mathbf{T}_l
    -2\delta_{ij}\delta_{j\ell}\mathbf{T}_i\cdot\mathbf{T}_k
    -2(\delta_{ik}\delta_{kl}+\delta_{jk}\delta_{kl})\mathbf{T}_i\cdot\mathbf{T}_j
    \big)\,.
    \label{eq:colour_id_2}
    \end{split}
\end{align}
\fi

has been used in the derivation of \eqn{eq:qqg_eikonal_quadrupole}.
The both can straightforwardly be proven using
%
\begin{align}
    {\bf{T}}_i^{a}{\bf{T}}_j^{b}=
    {\bf{T}}_j^{b}{\bf{T}}_i^{a}
    + if^{a b c}\delta_{ij}{\bf{T}}_i^{c}\,.
\end{align}





==> app_so_sc.tex <==
\section{Strongly-ordered soft limits of tree-level splitting amplitudes}
\label{app:so_collinear}
In this appendix we study the multiple collinear limit of the $q\bar{q}g$ strongly-ordered soft factorisation formulae. Below, we will use that the quadrupole operator is exact in the strongly-ordered limits, 
%
\begin{align}
    \mathscr{S}_{3}\,\mathcal{U}_{(\text{quad.})}^{q\bar{q}g} =
    \mathscr{S}_{12}\,\mathcal{U}_{(\text{quad.})}^{q\bar{q}g} \equiv
    \mathcal{U}_{(\text{quad.})}^{q\bar{q}g}\,.
\end{align}
%
The explicit form of $\mathcal{U}_{(\text{quad.})}^{q\bar{q}g}$ is shown in eq.~\eqref{eq:sc_quad}. \rayan{We will write our results in a more compact form by making use of both the dipole and charge conjugation symmetry under the exchanges $(i\leftrightarrow j)$ and $(1\leftrightarrow 2)$, respectively.
}

\iffalse
 We will routinely exploit this (as well as the symmetry under the exchange of the quark momenta $p_1$ and $p_2$) to express our results in a more compact form. For example, we may write the dipole eikonal factor as,
    %
    \begin{align}
        Q_{ij}^{q\bar{q}g}(p_1,p_2,p_3) = 
        Q_{ij}^{q\bar{q}g\,\,\text{symm.}}(p_1,p_2,p_3) +
        %Q_{(ij)}^{q\bar{q}g}(q_{(1},q_{2)},p_3)
        \begin{pmatrix}
        1 \leftrightarrow 2 \\
        i \leftrightarrow j
        \end{pmatrix}\,,
        %Q_{(ij)}^{q\bar{q}g} + (i \leftrightarrow j)\,,
    \end{align}
    %
    %where we introduced the notation $(ij)$ to denote the reduced expression.
    where we introduced the superscript ``symm." to denote the reduced expression.
\fi

First, we consider the simplest case of two soft gluons within a collinear set where $p_{12} \ll p_3$. We obtain the following factorisation formula,
%
\begin{align}
\begin{split}
& \mathscr{S}_{12}\,\mathscr{S}_{123}
\left[\left(\frac{2\mu^{2\eps}g_s^2}{s_{1\ldots m}}\right)^{m-1}\hat{P}_{\bar{q}_1 p_2g_3f_4\ldots f_m}^{ss'}\right]
= (\mu^{2\eps}g_s^2)^3
\mathcal{T}^{ss'}_{ff_{m+1}\ldots f_n}
\frac{1}{\mathcal{C}_{f}}
\left(
\mathscr{S}_{12}\,\mathcal{U}_{(\text{dip.})}^{q\bar{q}g}
%+\mathscr{S}_{12}\,\mathcal{U}_{(\text{trip.})}^{q\bar{q}g}
+\mathcal{U}_{(\text{quad.})}^{q\bar{q}g}
\right)\,,
\end{split}
\label{eq:P_soft_qqg_so12}
\end{align}
%
The quantity $\mathscr{S}_{12}\,\mathcal{U}_{(\text{dip.})}^{q\bar{q}g}$ is equivalent to eq.~\eqref{eq:sc_dipole} up to replacing ${U}_{ij;123}^{q\bar{q}g}$ by its strongly-ordered approximation, given by
%
\begin{align*}
%\begin{split}
%CHECKED
    &\mathscr{S}_{12}\,{U}_{ij;123}^{q\bar{q}g}(p_1,p_2,p_3)\\ &\,\,\,= 
    \mathscr{S}_{12}\,Q_{ij}^{q\bar{q}g\,\,\text{symm.}}(p_1,p_2,p_3)
    %u_{0\,(\text{dip.})}
    +T_R C_A \frac{1}{s_{3(12)}^2}
    \bigg\{\frac{2z_2^2s_{13}+2z_1^2s_{23}}{z_3s_{12}^2z_{12}}+\frac{D-6}{2s_{12}}\left( 
    1
    %-u_{i\,(\text{dip.})}
    -\frac{4z_1}{z_{12}}
    \right) \\
        &\,\,\,+ \frac{4}{z_{12}}\bigg[
    \frac{1}{s_{12}^2s_{i(12)}}\left(
    \frac{z_1}{s_{3i}}\left(
    \frac{4s_{23}z_i\left(s_{13}s_{2i}-s_{1i}s_{23}\right)}{z_3}-s_{13}s_{2i}^2-s_{1i}^2s_{23}
    \right) \right. \numberthis\\
    &\,\,\,+\left.
    \frac{2z_is_{12}s_{3(12)}}{z_3}\left( 
    \frac{z_3s_{1i}-s_{13}z_i}{s_{3i}}+z_1\right)
    \right)
    -\frac{z_1^2s_{23}}{z_3s_{12}^2}
    \bigg]
    \bigg\}
    +\begin{pmatrix}
        1 \leftrightarrow 2 \\
        i \leftrightarrow j
    \end{pmatrix}
    %-u_{j\,(\text{dip.})}
%\end{split}
\end{align*}
%
\rayan{where $\mathscr{S}_{12}\,Q_{ij}^{q\bar{q}g\,\,\text{symm.}}$ is the symmetrised expression extracted from the right-hand side of  eq.~\eqref{eq:so12_nab}.}
\rayan{the problem with removing the definition for the symmetrised dipole factors from the main text, e.g. $\mathscr{S}_{12}\,Q_{ij}^{q\bar{q}g\,\,\text{symm.}}$, is that their reference here becomes very clumsy.}
The three-parton correlated part is power-suppressed in the limit where the momentum of the $q\bar{q}$ pair is much softer than that of the on-shell gluon, i.e. $\mathscr{S}_{12}\,\mathcal{U}_{(\text{trip.})}^{q\bar{q}g}=0$ to leading order. Therefore, it does not contribute to eq.~\eqref{eq:P_soft_qqg_so12}.

Next, we investigate the case where $p_3 \ll p_{12}$. The factorisation formula is given by,
%
\begin{align}
\begin{split}
& \mathscr{S}_{3}\,\mathscr{S}_{123}
\left[\left(\frac{2\mu^{2\eps}g_s^2}{s_{1\ldots m}}\right)^{m-1}\hat{P}_{\bar{q}_1 p_2g_3f_4\ldots f_m}^{ss'}\right]
\\  &\qquad
= (\mu^{2\eps}g_s^2)^3
\mathcal{T}^{ss'}_{ff_{m+1}\ldots f_n}
\frac{1}{\mathcal{C}_{f}}
\left(
\mathscr{S}_{3}\,\mathcal{U}_{(\text{dip.})}^{q\bar{q}g}
+\mathscr{S}_{3}\,\mathcal{U}_{(\text{trip.})}^{q\bar{q}g}
+\mathcal{U}_{(\text{quad.})}^{q\bar{q}g}
\right)\,.
\end{split}
\label{eq:P_soft_qqg_so3}
\end{align}
%
The quantity $\mathscr{S}_{3}\,\mathcal{U}_{(\text{dip.})}^{q\bar{q}g}$ is equivalent to eq.~\eqref{eq:sc_dipole} up to replacing ${U}_{ij;123}^{q\bar{q}g}$ by its strongly-ordered approximation in which $p_3\ll p_{12}$. The abelian part factorises in terms of the $q\bar{q}$ eikonal function times a simple kinematic factor $s_{12}/(s_{13}s_{23})\sim\lambda_c^{-2}\lambda_s^{-4}$. Thus, the scaling behavior is determined solely by $Q_{ij}^{q\bar{q}}$, and it is straightforward to calculate the collinear limit as,
%
\begin{align}
%CHECKED
    \mathscr{S}_{3}\,{U}_{ij;123}^{q\bar{q}g\,(\text{ab})}(p_1,p_2,p_3) =
    \frac{4s_{12}}{s_{13}s_{23}}\mathscr{C}_{1\ldots m}\, Q_{ij}^{q\bar{q}}(p_1,p_2)\,,
\end{align}
%
where we extract the leading divergent term of $\mathcal{O}(\lambda_c^{-4}\lambda_s^{-4})$,
%
\begin{align}
\begin{split}
%CHECKED
    &\mathscr{C}_{1\ldots m}\, Q_{ij}^{q\bar{q}}(p_1,p_2) \\
    &\,\,\,=
    Q_{ij}^{q\bar{q}}(p_1,p_2)+
    \frac{4}{s_{12}^2z_{12}}\left(\frac{2z_1z_2}{z_{12}}
    +\frac{s_{12}z_i-z_2s_{1i}-z_1s_{2i}}{s_{i(12)}}
    +\frac{s_{12}z_j-z_2s_{1j}-z_1s_{2j}}{s_{j(12)}}
    \right)
\end{split}
\end{align}
%
The non-abelian factor is slightly more lengthy,
%
\begin{align}
\begin{split}
%CHECKED
    &\mathscr{S}_{3}\,{U}_{ij;123}^{q\bar{q}g\,(\text{nab})}(p_1,p_2,p_3) \\
    &\,\,\,= 
    \mathscr{S}_{3}\,{Q}^{q\bar{q}g\,(\text{nab})\,\,\text{symm.}}_{ij}(p_1,p_2,p_3)
    %u_{0\,(\text{dip.})}
    +\frac{4z_1z_2\left(z_2s_{13}-z_3s_{12}\right)}{z_3s_{12}^2z_{12}^2s_{13}s_{23}}
    %-u_{i\,(\text{dip.})}
     +\frac{4}{s_{i(12)}^2}\bigg\{
    \frac{s_{1i}s_{2i}}{s_{12}s_{13}s_{23}} \\
    &\,\,\,+\frac{1}{z_{12}}\bigg[
    \frac{1}{z_3s_{3i}s_{12}}\left(
    \frac{z_is_{i(12)}\left(z_3s_{2i}+z_2s_{3i}\right)}{s_{23}}
    -z_i^2s_{i(12)}
    \right)
    -\frac{z_is_{i(12)}}{s_{13}s_{23}}\\
    &\,\,\,+\frac{z_2s_{1i}^2+z_1s_{2i}^2}{s_{23}}\left( \frac{1}{s_{13}s_{12}} -\frac{z_2}{z_3s_{12}^2}\right) 
    \bigg]
    +\frac{1}{s_{12}^2z_{12}^2}\left[
    \frac{(s_{1i}z_2-s_{2i}z_1)^2}{s_{3i}}\left(\frac{z_i}{z_3}-\frac{s_{2i}}{s_{23}}\right) \right.\\
    &\,\,\,-\left.
    \frac{s_{2i}^2s_{1i}z_{12}^2}{s_{23}s_{3i}}
    \right] 
    \bigg\}
    %-u_{j\,(\text{dip.})}
    +\begin{pmatrix}
        1 \leftrightarrow 2 \\
        i \leftrightarrow j
    \end{pmatrix}\,,
\end{split}
\end{align}
%
where the explicit form of $\mathscr{S}_{3}\,{Q}^{q\bar{q}g\,(\text{nab})\,\,\text{symm.}}_{ij}$ is given in eq.~\eqref{eq:so3_nab}.

Finally, the strongly-ordered tripole factor in eq.~\eqref{eq:P_soft_qqg_so3} reads,
%
\begin{align*}
%CHECKED
%    \begin{split}
    &\mathscr{S}_{3}\,{U}_{ijk;123}^{q\bar{q}g}(p_1,p_2,p_3) \\&\,\,\,= 
    \mathscr{S}_{3}\,Q_{ijk}^{q\bar{q}g}(p_1,p_2,p_3) +
    \frac{8T_R}{s_{12}^2} \bigg\{
    \frac{z_1}{z_3s_{13}}\frac{s_{12}s_{ik}-s_{1i}s_{2k}-s_{1k}s_{2i}}{s_{i(12)}s_{k(12)}} 
    +\frac{1}{z_{12}s_{13}}\left(\frac{s_{1j}}{s_{3j}}-
    \frac{z_1}{z_3}\right)
    \\
    &\,\,\,\times\,\left(
    \frac{2z_1z_2}{z_{12}}
    -\frac{z_2s_{1i}+z_1s_{2i}-s_{12}z_i}{s_{i(12)}}
    -\frac{z_2s_{1k}+z_1s_{2k}-s_{12}z_k}{s_{k(12)}}
    \right)
    \bigg\}\,, \numberthis
%    \end{split}
\end{align*}
%
where $\mathscr{S}_{3}\,Q_{ijk}^{q\bar{q}g}$ is defined in eq.~\eqref{eq:Q_trip_so3}

In the simplest case of a strongly-ordered triple soft limit within the quadruple collinear splitting $f \to \bar{q}_1 p_2 g_3 f_4$ we obtain the analogues of eq.~\eqref{eq:Split4_qqg_soft},
%
\begin{align}
\label{eq:Split4_qqg_soft_so12}
    &\mathscr{S}_{12}\, \mathscr{S}_{123}
\left[\left(\frac{2\mu^{2\eps}g_s^2}{s_{1\ldots m}}\right)^{m-1}\hat{P}_{\bar{q}_1 p_2g_3f_4}^{ss'}\right]
= (\mu^{2\eps}g_s^2)^3
\left(
C_4 \mathscr{S}_{12}\,U_{44;123}^{q\bar{q}g}
+ 2C_4^2 U_{4444;123}^{q\bar{q}g}
\right)
%|\mathcal{M}_{f_4\ldots f_n}|^2
\delta^{ss'}\,,
\end{align}
%
and
%
\begin{align}
\label{eq:Split4_qqg_soft_so3}
    &\mathscr{S}_{3}\, \mathscr{S}_{123}
\left[\left(\frac{2\mu^{2\eps}g_s^2}{s_{1\ldots m}}\right)^{m-1}\hat{P}_{\bar{q}_1 p_2g_3f_4}^{ss'}\right]
\\ \nonumber &\,\,\, 
= (\mu^{2\eps}g_s^2)^3
\left[
C_4 \mathscr{S}_{3}\,U_{44;123}^{q\bar{q}g} + \left(4C_F^2-\frac{3}{2}C_A C_F\right)\delta_{f_4 q_4} \mathscr{S}_{3}\,U_{444;123}^{q\bar{q}g}
+ 2C_4^2 U_{4444;123}^{q\bar{q}g}
\right]
%|\mathcal{M}_{f_4\ldots f_n}|^2
\delta^{ss'}\,.
\end{align}
%
The explicit form of $U_{4444;123}^{q\bar{q}g}$ is given in eq.~\eqref{eq:U_quad_4split}. Again, we have checked the validity of eqs.~\eqref{eq:Split4_qqg_soft_so12} and \eqref{eq:Split4_qqg_soft_so3} for the relevant cases shown in eqs.~\eqref{eq:q_split} and \eqref{eq:g_split}. This is both a strong check on the splitting amplitudes themselves, and on the results for the $U$ factors. 


==> app_tripole.tex <==
\section{Three-parton colour correlated soft function}
\label{app:tripole}
In this appendix we show the calculation for the tripole colour correlated contribution. It will be convenient to write eq.~\eqref{eq:W_current} as,
%
\begin{align}
    \mathbf{W}^{a,\mu}(q_1,q_2,q_3) &=
    \mathbf{w}_1^{a,\mu} + \mathbf{w}_2^{a,\mu}\,,
\end{align}
%
where
%
\begin{align}
    \mathbf{w}_1^{a,\mu} &=
    \sum_i
    \mathbf{J}_i^{b,\nu}(q_{123})\,
    \frac{1}{s_{123}} \left[
     \frac{1}{s_{13}}\gamma_\nu \slashed{p}_{13}\gamma^\mu \left(t^b t^a \right)
     -
     \frac{1}{s_{23}}\gamma^\mu \slashed{p}_{23}\gamma_\nu \left(t^a t^b \right)
     \right]\,, \\
    \begin{split}
     \mathbf{w}_2^{a,\mu} &=
     \sum_i
    \mathbf{J}_i^{b,\nu}(q_{123})\,
     \frac{i}{s_{12}}f^{abc}\left[\frac{1}{2}\delta_{\nu}{}^\alpha
     \left(\mathcal{S}_{i}^\mu(q_{3})-\mathcal{S}_{i}^\mu(q_{12})\right) + \frac{1}{s_{123}}U_\nu{}^{\alpha\mu}(q_{12},q_3)\right]\gamma_\alpha t^c\,.
    \end{split}
\end{align}
%
Interference between the soft current $\mathbf{K}$, defined in eq.~\eqref{eq:K_current}, and $\mathbf{w}_1$ yields both dipole colour correlations proportional to $C_A$ and irreducible colour correlations between three hard partons. Explicitly, we have 
\rayan{not sure about overall sign for $C_A$ part, which I think depends on whether I have $\left\{\mathbf{T}_i^a,\mathbf{T}_j^c\right\}$ or $\left\{\mathbf{T}_i^c,\mathbf{T}_j^a\right\}$?}
\begin{align}
\begin{split}
    [\mathbf{K}^{a,\mu}&(q_1,q_2,q_3)]^*
    d_{\mu\nu}(q_3,n)
    \mathbf{w}^{a,\nu}(q_1,q_2,q_3)
    +\text{c.c.} \\ &=
    \frac{1}{s_{12}s_{123}}\sum_{i,j,k}
    \frac{1}{2}
    \left\{\mathbf{T}_i^a,\mathbf{T}_j^c\right\}\mathbf{T}_k^b 
    \left(
    \Tr\left(t^c t^a t^b\right)  %+\mathbf{T}_k^b\left\{\mathbf{T}_i^c,\mathbf{T}_j^a\right\}\,\text{tr}\left(t^b t^a t^c\right) 
    \Pi^{(1)}_{\alpha\beta\mu}(q_1,q_2,q_3) \right.\\
    &-\left.\Tr\left(t^c t^b t^a\right)
    \Pi^{(2)}_{\alpha\beta\mu}(q_1,q_2,q_3)
    \right)
    \mathcal{S}_i^\alpha(q_{12})
    \mathcal{S}_j^\mu(q_{3})
    \mathcal{S}_k^\beta(q_{123})
    +\text{c.c.} \\
    &+\ldots\,.
\label{eq:tripole}
\end{split}
\end{align}
%
The ellipses denote terms that vanish by colour conservation, and can thus be neglected. They have their origin in longitudinal polarisations proportional to either $q_3^\mu$ or $q_3^\nu$.
The kinematic factors on the rigth-hand side in eq.~\eqref{eq:tripole} have the explicit form,
%
\begin{align}
    \Pi^{(1)}_{\alpha\beta\mu}(q_1,q_2,q_3) =
    \frac{1}{s_{23}}
    \Tr\left(
    \gamma_\alpha\slashed{q}_2\gamma_\mu\slashed{q}_{23}\gamma_\beta\slashed{q}_1 
    \right)\,, \\
    \Pi^{(2)}_{\alpha\beta\mu}(q_1,q_2,q_3) =
    \frac{1}{s_{13}}
    \Tr\left(
    \gamma_\alpha\slashed{q}_2\gamma_\beta\slashed{q}_{13}\gamma_\mu\slashed{q}_1 
    \right)\,.
\end{align}
%
Note that under the exchange $(1\leftrightarrow 2)$ they satisfy the following relation,
%
\begin{align}
    \Pi^{(1)}_{\alpha\beta\mu}(q_1,q_2,q_3) =
    \Pi^{(2)}_{\alpha\beta\mu}(q_2,q_1,q_3)\,.
\end{align}
%
To evaluate eq.~\eqref{eq:tripole}, we use the colour identity
%
\begin{align}
    \Tr\left(t^a t^b t^c\right) = 
    \frac{1}{4}\left(d^{abc}+if^{abc}\right)\,.
\end{align}
%
As a result we obtain,
\rayan{up to overall sign for the $f^{abc}$ term which I'm unsure about now...}
%
\begin{align}
\begin{split}
    -[\mathbf{K}^{a,\mu}&(q_1,q_2,q_3)]^\dagger
    g_{\mu\nu} 
    \mathbf{w}^{a,\nu}(q_1,q_2,q_3)
    +\text{c.c.} \\ &=
    -\frac{1}{8s_{12}s_{123}}\sum_{i,j,k}
    \mathcal{S}_i^\alpha(q_{12})
    \mathcal{S}_j^\mu(q_{3})
    \mathcal{S}_k^\beta(q_{123}) \Big\{
    if^{abc}\left[\left\{\mathbf{T}_i^a,\mathbf{T}_j^b\right\},\mathbf{T}_k^c\right] \\
    &\times\left(\Pi^{(1)}_{\alpha\beta\mu}(q_1,q_2,q_3) 
    +\Pi^{(2)}_{\alpha\beta\mu}(q_1,q_2,q_3) \right)
    +d^{abc}\left\{\left\{\mathbf{T}_i^a,\mathbf{T}_j^b\right\},\mathbf{T}_k^c\right\} \\
    &\times
    \left(\Pi^{(1)}_{\alpha\beta\mu}(q_1,q_2,q_3) 
    -\Pi^{(2)}_{\alpha\beta\mu}(q_1,q_2,q_3) \right)
    \Big\}\,.
\end{split}
\end{align}
%
Next, we have that
%
\begin{align}
    if^{abc}\left[\left\{\mathbf{T}_i^a,\mathbf{T}_j^b\right\},\mathbf{T}_k^c\right] &=
    2C_A \left(\mathbf T_i \cdot \mathbf T_j\right)(\delta_{ik}-\delta_{jk})\,, \\
    d^{abc}\left\{\left\{\mathbf{T}_i^a,\mathbf{T}_j^b\right\},\mathbf{T}_k^c\right\}&=
    4d^{abc}\,\mathbf{T}_i^a\mathbf{T}_j^b\mathbf{T}_k^c\,.
\end{align}
%
Notice the relative sign difference between the kinematic terms multiplying the symmetric colour factor $d^{abc}$.
